LLM4VG: Large Language Models Evaluation for Video Grounding

Recently, researchers have attempted to investigate the capability of LLMs in handling videos and proposed several video LLM models. However, the ability of LLMs to handle video grounding (VG), which is an important time-related video task requiring the model to precisely locate the start and end timestamps of temporal moments in videos that match the given textual queries, still remains unclear and unexplored in literature. To fill the gap, in this paper, we propose the LLM4VG benchmark, which systematically evaluates the performance of different LLMs on video grounding tasks. Based on our proposed LLM4VG, we design extensive experiments to examine two groups of video LLM models on video grounding: (i) the video LLMs trained on the text-video pairs (denoted as VidLLM), and (ii) the LLMs combined with pretrained visual description models such as the video/image captioning model. We propose prompt methods to integrate the instruction of VG and description from different kinds of generators, including caption-based generators for direct visual description and VQA-based generators for information enhancement. We also provide comprehensive comparisons of various VidLLMs and explore the influence of different choices of visual models, LLMs, prompt designs, etc, as well. Our experimental evaluations lead to two conclusions: (i) the existing VidLLMs are still far away from achieving satisfactory video grounding performance, and more time-related video tasks should be included to further fine-tune these models, and (ii) the combination of LLMs and visual models shows preliminary abilities for video grounding with considerable potential for improvement by resorting to more reliable models and further guidance of prompt instructions.

==> backup/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

With the rapid development of large language models (LLM) in recent years, various artificial intelligence tasks beyond natural language processing, such as dynamic graphs~\cite{zhang2023llm4dyg}, visual question answering~\cite{guo2023images}, reinforcement learning~\cite{10.5555/3618408.3618558}, have begun to expand into this field. One particularly important and closely related field to human life is visual and audio data, which is a focal point for achieving human-computer interaction~\cite{mackenzie2012human}, and more and more tasks requiring visual and audio features are dedicated to linking LLM's word processing capabilities with visual and auditory perception abilities~\cite{lyu2023macaw,zhao2023learning}. Videos, compared to visual images, possess richer temporal information, making them more relevant to human daily life and occupying a more important position in the field of artificial intelligence~\cite{camastra2015machine,redmon2016you,han2023h2v4sports}.  In order to utilize the language understanding, analysis, reasoning abilities, and common sense knowledge of LLM, several groundbreaking works have been used to introduce LLM in the visual and audio fields~\cite{guo2023images,Maaz2023VideoChatGPT,chen2023videollm,damonlpsg2023videollama}. Such surveys may reveal a wider range of video data applications.



% On the one hand, through additional time dimensions, LLM can explain and understand the changes and relationships of video content frame by frame, and mine information that single-frame images do not have~\cite{tan2023towards}. On the other hand, there are additional research challenges for capturing and understanding video or image features and transforming them into textual language~\cite{aradhye2009video2text}, also, evaluating LLM's ability to understand spatiotemporal changes in video content is crucial for its application in the video field~\cite{feng2023multimedia}.

% The daily living environment of the world seen by us humans or visually capable machines can be understood as a continuously changing video scene, providing a vast amount of valuable data for humans and intelligent agents to receive, analyze, and make decisions~\cite{vasudevan2018object}.

% For example, on artificial intelligence tasks such as in indoor robot navigation and positioning, in the decision-making stage, the intelligent agent will continuously make actions while receiving video information, and in the information perception stage, the received external video content will keep updated over time.

Although LLMs have been widely applied in various fields, including video, their application in video grounding tasks still remains unexplored in literature,  which raises our attention.  As a task that connects video content with language narration and spatiotemporal perception, video grounding requires intelligence to output a time period corresponding to a caption for the video~\cite{wang2022video}. During the open environment of our reality, the performance of LLMs on video grounding will directly determine their spatiotemporal perception ability of external objects~\cite{feng2023multimedia}, which is crucial for achieving human-computer interaction.


% Video grounding was first conceptualized as a cross-modal artificial intelligence task in the past decade~\cite{gao2017tall}, which has made significant progress in both academia and industry in recent years. As it stands today, video grounding has been comprehensively described as a connection between videos and description statements to output a time period corresponding to a caption for the video~\cite{wang2022video}. Summarized as grounding actions and objects by language in videos, video grounding generally consists of two parts, which are temporary activity localization by language~\cite{gao2017tall,anne2017localizing} (i.e., given a query containing an activity description, find the start and end times of the corresponding action or event) and spatio temporary object referencing by language~\cite{yamaguchi2017spatio,vasudevan2018object} (i.e., given a query containing an object description, find continuous bounding boxes in time and space). 




However, the task that LLMs solving video grounding is non-trivial with the challenges as follows: 1) How to design tasks of video grounding for LLMs to simultaneously accept and understand the audio-visual information of the video and the textual information of the grounding problem, and conduct reasoning and analysis; 2) How to design the prompts for video grounding tasks, where the image frames and audio information of videos that cannot be directly processed by most LLMs should be taken into consideration in natural language; 3) How to establish effective evaluation dimension to further improve LLMs' ability to understand and handle video grounding tasks.

% However, the problem that LLM solves video grounding tasks still remains unexplored in literature, and is non-trivial with the challenges as follows: 1) How to design tasks of video grounding for LLMs to simultaneously accept and understand the audio-visual information of the video and the textual information of the grounding problem, and conducting reasoning and analysis; 2) How to design the prompts for video grounding tasks, where the image frames and audio information of videos that cannot be directly processed by most LLMs should be taken into consideration in natural language; 3) How to establish effective evaluation dimension to further improve LLMs' ability to understand and handle video grounding tasks.

To this end, in this paper, we propose to explore the following research question, is LLM able to understand spatial-temporal information and conduct language analysis on video grounding via natural language?

To address these issues, we further propose LLM4VG, a comprehensive benchmark for evaluating the temporal understanding and semantic reasoning analysis capabilities of LLMs on video grounding tasks. In this work, we use a method of converting video content to text description, and introduce a combination of visual description model and LLMs for video grounding, so that normal LLMs can access and handle video grounding tasks. More importantly, we also systematically evaluated and analyzed the video grounding results of different LLMs combined with different visual description models and promoting methods. 

With this paper, we make the following contributions.
\begin{itemize}
    \item We propose LLM4VG, a comprehensive benchmark that systematically evaluates the performance of video grounding tasks for large language models. We have adopted two methods to complete video grounding. One is to use the existing VideoLLMs to directly accept the video content and video grounding task instructions and output the prediction results. We also introduce a method of converting video content to text description with visual description generators for normal LLMs, which bridges the visual data and language content.
    
    \item LLM4VG allows normal LLMs to access and handle video grounding tasks, which enables LLMs to perform zero-shot and one-shot video grounding without costly extra pre-training, making low-cost deployment of LLM for video grounding possible.

    \item We analyzed the influences of applying \textbf{six} visual models, \textbf{three} LLMs, and \textbf{three} prompting methods, comparing them with \textbf{three} VideoLLMs which were directly instructed to conduct video grounding tasks, and we concluded fine-grained observations about LLMs on video grounding. 
    
    
\end{itemize}

The results we observe present the \textbf{conclusion} that our method connecting LLMs and visual models has higher ability of temporal understanding than VideoLLMs, showing preliminary abilities for video grounding tasks, but they are both still far from satisfying the current video grounding tasks. It demonstrates that more temporal-related video tasks should be added to further finetune the VideoLLMs. As for the combination of visual models and LLMs, their video grounding ability is largely limited to the performance of the prompt designs and visual description models. The prompting method of instructing LLMs to separately judge the predictability and infer can significantly improve the performance of video grounding. More fine-grained visual models are also required to introduce more visual information to further help LLMs understand the visual scene and complete the video grounding task.
% The evaluation results we observe lead to the following findings with LLM4VG:
% \begin{itemize}
%     \item \textbf{LLMs show preliminary abilities for video grounding tasks, outperforming the videoLLMs.} The results we observe present that our method connecting LLMs and visual models shows higher ability of temporal understanding than VideoLLMs, outperforming 
% \end{itemize}

% 未完
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figure/framework.pdf}
    \caption{Framework of video grounding for LLMs. (a) stands for video grounding with VideoLLMs. (b) stands for video grounding with LLMs and visual models. The dashed box represents that in the one-shot method, we will input exemplar prompt, description prompt, and question prompt, while in the zero-shot method, we will not input exemplar prompt.}
    \label{fig:framework}
\end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figure/framework2.pdf}
%     \caption{Framework of video grounding for VideoLLM that can directly access video data.}
%     \label{fig:framework-videollm}
% \end{figure}

\section{Related Work}
\subsection{LLMs for Tasks with Videos}
% aimed at understanding and generating human language~\cite{brown2020language,zhang2022opt}

Large Language Model (LLM) is a type of artificial intelligence model trained through massive text data~\cite{radford2018improving}, and it is able to perform a wide range of tasks including text summarization, translation, reasoning, emotional analysis, and more~\cite{kojima2022large,zhou2022least,min2023recent}.  with the introduction of GPT-3~\cite{floridi2020gpt},  InstructGPT~\cite{ouyang2022training}, and GPT-4~\cite{gpt4}, this concept has become widely known for understanding and generating human language.

% Its unique characteristic compared to traditional natural language processing models is the extremely large scale with billions of parameters, allowing the LLM to better learn and analyze the complex patterns of language data, outperforming the past natural language processing models~\cite{}.

However, in the digital world today, video and audio content share the same importance with textual content as part of multimedia data~\cite{zhu2020multimedia}. This makes it hard for a simple LLM to expand into the field of audiovisual perception to meet the needs of users. To address this issue, two different approaches have been proposed in the academic community. One is to develop a large language model with multimodal information processing capabilities. Therefore, many large language models that can handle videos have emerged, such as Video-LLaMA~\cite{damonlpsg2023videollama}, Video-Chat~\cite{2023videochat} and Video-ChatGPT~\cite{Maaz2023VideoChatGPT}. We collectively refer to them as VideoLLM~\cite{chen2023videollm}. While retaining LLM's powerful language comprehension abilities, VideoLLM has also demonstrated impressive ability in receiving and understanding visual and auditory content. The other one is to convert the visual and audio information into intermediate language descriptions instead of dense vectors, using the descriptions and few-shot in-context exemplars to instruct normal LLMs to complete video-related tasks, which has been used by Guo et al. for visual question answering tasks of LLMs~\cite{guo2023images}.


 Naturally, we wonder whether the method mentioned above can complete cross-modal artificial intelligence tasks related to video, such as video grounding. 

% \subsection{LLMs for other related tasks}

\subsection{Video Grounding}

Video grounding is a task that requires intelligence to localize the starting and ending times of the segment target from a video~\cite{chen2018temporally}, which has drawn increasing attention over the past few years~\cite{lan2023survey}, since video grounding task is closely related to quite a few computer vision and language processing methods such as video understanding, video retrieval, and human-computer interaction, etc~\cite{yuan2021closer,gabeur2020multi}.

% such as difficulty in establishing connections between language descriptions and complex video content, and difficulty in accurately locating video content in complex backgrounds,
% Xu et al.~\cite{xu2019multilevel} proposed to integrate the query and neural network to generate query-guided proposals, which improve the quality of the proposals.
Regarding the challenges of video grounding tasks,  many approaches have been proposed~\cite{zeng2020dense,chen2023curriculum,xu2019multilevel}. He et al. propose a reinforcement learning method that includes an adjustable temporal window with a sliding boundary, which has the learned policy for video grounding~\cite{he2019read}.  Zeng et al. proposed a dense regression network that regresses the distances from every frame to the starting or ending frame of the video segment described by the query~\cite{zeng2020dense}. Chen et al. proposed an Adaptive Dual-branch Promoted Network (ADPN) that exploits consistency and complementarity of audio and visual information instead of focusing on visual information only~\cite{chen2023curriculum}. These methods, however, all require the use of annotated specific video grounding training datasets for pre-training, which cannot be directly applied to task scenarios, and their generalization ability to solve video grounding problems in open environments is also difficult to guarantee.
% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.


